Scalable Inference of System-level Models from Component Logs

Behavioral software models play a key role in many software engineering tasks; unfortunately, these models either are not available during software development or, if available, they quickly become outdated as the implementations evolve. Model inference techniques have been proposed as a viable solution to extract finite-state models from execution logs. However, existing techniques do not scale well when processing very large logs, such as system-level logs obtained by combining component-level logs. Furthermore, in the case of component-based systems, existing techniques assume to know the definitions of communication channels between components. However, this information is usually not available in the case of systems integrating 3rd-party components with limited documentation. In this paper, we address the scalability problem of inferring the model of a component-based system from the individual component-level logs, when the only available information about the system are high-level architecture dependencies among components and a (possibly incomplete) list of log message templates denoting communication events between components. Our model inference technique, called SCALER, follows a divide and conquer approach. The idea is to first infer a model of each system component from the corresponding logs; then, the individual component models are merged together taking into account the dependencies among components, as reflected in the logs. We evaluated SCALER in terms of scalability and accuracy, using a dataset of logs from an industrial system; the results show that SCALER can process much larger logs than a state-of-the-art tool, while yielding more accurate models.

==> figures/logs.tex <==
\centering
\resizebox{0.7\linewidth}{!}{
\setlength\tabcolsep{1mm}
\begin{tabular}{ |c|l|l| }
\hline
{Comp} & {Execution-1}& {Execution-2}\\
\hline
\textit{TC} & \begin{tabular}[]{@{\ttfamily}l@{}}
$e_{1,1}^{\mathit{TC}}=$14:26:01 sending X via f0\\ 
$e_{2,1}^{\mathit{TC}}=$14:26:02 TC accepted
\end{tabular} & \begin{tabular}[c]{@{\ttfamily}l@{}}
$e_{1,2}^{\mathit{TC}}=$14:30:11 sending Y via f1 \\ 
$e_{2,2}^{\mathit{TC}}=$14:30:12 wait message\end{tabular} \\
\hline
\textit{MUX} & \begin{tabular}[]{@{\ttfamily}l@{}}
$e_{1,1}^{\mathit{MUX}}=$14:26:01 initialize\\
$e_{2,1}^{\mathit{MUX}}=$14:26:01 commandName = X\\
$e_{3,1}^{\mathit{MUX}}=$14:26:01 commandName = X\\
$e_{4,1}^{\mathit{MUX}}=$14:26:01 data flow ID = f0\\
$e_{5,1}^{\mathit{MUX}}=$14:26:02 send = ok
\end{tabular} & \begin{tabular}[c]{@{\ttfamily}l@{}}
$e_{1,2}^{\mathit{MUX}}=$14:30:11 initialize\\
$e_{2,2}^{\mathit{MUX}}=$14:30:12 commandName = Y\\
$e_{3,2}^{\mathit{MUX}}=$14:30:12 data flow ID = f1\\
$e_{4,2}^{\mathit{MUX}}=$14:30:12 send = no
\end{tabular} \\
\hline
\textit{GW} & $e_{1,1}^{\mathit{GW}}=$14:26:01 encrypt TC\_01 & $e_{1,2}^{\mathit{GW}}=$14:30:12 reject command \\
\hline
\textit{CHK} & \begin{tabular}[c]{@{\ttfamily}l@{}}
$e_{1,1}^{\mathit{CHK}}=$14:26:01 mode 1\\
$e_{2,1}^{\mathit{CHK}}=$14:26:02 automatic config
\end{tabular} & $e_{1,2}^{\mathit{CHK}}=$14:30:11 mode 0\\
\hline                                                                                                                                     
\end{tabular}}

